Active Continual Learning: On Balancing Knowledge Retention and Learnability

Acquiring new knowledge without forgetting what has been learned in a sequence of tasks is the central focus of continual learning (CL). While tasks arrive sequentially, the training data are often prepared and annotated independently, leading to the CL of incoming supervised learning tasks. This paper considers the under-explored problem of active continual learning (ACL) for a sequence of active learning (AL) tasks, where each incoming task includes a pool of unlabelled data and an annotation budget. We investigate the effectiveness and interplay between several AL and CL algorithms in the domain, class and task-incremental scenarios. Our experiments reveal the trade-off between two contrasting goals of not forgetting the old knowledge and the ability to quickly learn new knowledge in CL and AL, respectively. While conditioning the AL query strategy on the annotations collected for the previous tasks leads to improved task performance on the domain and task incremental learning, our proposed forgetting-learning profile suggests a gap in balancing the effect of AL and CL for the class-incremental scenario.

==> tables/fig-analysis.tex <==
% \begin{figure}
% \centering
% \begin{minipage}{.5\textwidth}
%   \centering
%   \includegraphics[scale=0.33]{figures/taskpred-newsgroup_er.pdf}
%   \captionof{figure}{Task prediction probability of ACL models with ER and entropy strategy on 20News
% (Class-IL)}
%   \label{taskpred-20news-entropy}
% \end{minipage}%
% \begin{minipage}{.4\textwidth}
%   \centering
%   \includegraphics[scale=0.33]{figures/jaccard-al.pdf}
%   \captionof{figure}{Jaccard coefficient between sequential and independent AL queries of ACL methods with ER.}
%   \label{fig:jaccard}
% \end{minipage}
% \end{figure}


% % \begin{figure}
% %      \centering
% %          \includegraphics[scale=0.35]{figures/jaccard-al.pdf}
% % \caption{Jaccard coefficient between sequential and independent AL queries of ACL methods with ER.}
% %      \label{fig:jaccard}
% % \end{figure}

==> tables/fig-asc-lca-all-tasks.tex <==
\begin{figure*}
     \centering
       \includegraphics[scale=0.4]{figures/all-lca-asc.pdf}
     
     \label{fig:asc-lca-all-tasks}
     \caption{Average LCA of AL curves through tasks on ASC dataset.}
\end{figure*}

==> tables/fig-forgetting-lca-appx.tex <==
\begin{figure*}
     \centering
     \begin{subfigure}{\textwidth}
         \centering
         \includegraphics[scale=0.35]{figures/forget-lca-asc.pdf}
         \caption{Forgetting rate and LCA of ACL methods on ASC (Domain-IL).}
     \end{subfigure}
     \begin{subfigure}{\textwidth}
         \centering
         \includegraphics[scale=0.35]{figures/forget-lca-newsgroup.pdf}
         \caption{Forgetting rate and LCA of ACL methods on 20News (Class-IL).}
     \end{subfigure}
     \begin{subfigure}{\textwidth}
         \centering
          \includegraphics[scale=0.35]{figures/forget-lca-newsgroup-task.pdf}
         \caption{Forgetting rate and LCA of ACL methods on 20News (Task-IL).}
     \end{subfigure}
     \label{fig:forgetting-all}
     %\caption{Forgetting rate and LCA of ACL on asc dataset}
\end{figure*}

==> tables/fig-newsgroup-lca.tex <==
\begin{figure*}
     \centering
     \begin{subfigure}{\textwidth}
         \centering
         \includegraphics[scale=0.4]{figures/newsgroup_random}
     \end{subfigure}
     \begin{subfigure}{\textwidth}
         \centering
         \includegraphics[scale=0.4]{figures/newsgroup_entropy}
     \end{subfigure}
     \begin{subfigure}{\textwidth}
         \centering
         \includegraphics[scale=0.4]{figures/newsgroup_min_margin}
     \end{subfigure}
     \begin{subfigure}{\textwidth}
         \centering
         \includegraphics[scale=0.4]{figures/newsgroup_badge}
     \end{subfigure}
     \begin{subfigure}{\textwidth}
         \centering
         \includegraphics[scale=0.4]{figures/newsgroup_embedding_kmeans}
     \end{subfigure}
%     \hfill
     \label{fig:20news-all}
     \caption{Forgetting rate and LCA of ACL on 20News dataset.}
\end{figure*}

==> tables/tab-data.tex <==

\begin{table*}[]
\centering
\scalebox{0.8}{
\begin{tabular}{lrrrr}
 \toprule
 Domains &  train sents & dev sents & test sents \\
\midrule
Video Games & 4000 & 500 & 500 \\
Toys and Games & 4000 & 500 & 500 \\
Tools and Home Improvement & 4000 & 500 & 500 \\
Sports and Outdoors & 4000 & 500 & 500 \\
Pet Supplies & 4000 & 500 & 500 \\
Patio Lawn and Garden & 2952 & 500 & 369 \\
Office Products & 4000 & 500 & 500 \\
Musical Instruments & 2374 & 500 & 297 \\
Movies and TV & 4000 & 500 & 500 \\
Kindle Store & 4000 & 500 & 500 \\
 \bottomrule
\end{tabular}
}
\caption{DSC dataset - domain incremental}
\label{tab:data-dsc}
\end{table*}


\begin{table*}[]
\centering
\scalebox{0.8}{
\begin{tabular}{lrrrr}
 \toprule
 Task & Class &  train sents & dev sents & test sents \\
\midrule
0 & comp.graphics   & 800  & 100  & 100 \\
 & comp.os.ms-windows.misc   & 800  & 100  & 100 \\
\midrule
 1 & comp.sys.ibm.pc.hardware   & 800  & 100  & 100 \\
 & comp.sys.mac.hardware   & 800  & 100  & 100 \\
\midrule
 2 & comp.windows.x   & 800  & 100  & 100 \\
 & rec.autos   & 800  & 100  & 100 \\
\midrule
 3 & rec.motorcycles   & 800  & 100  & 100 \\
 & rec.sport.baseball   & 800  & 100  & 100 \\
\midrule
 4 & rec.sport.hockey   & 800  & 100  & 100 \\
 & sci.crypt   & 800  & 100  & 100 \\
\midrule
 5 & sci.electronics   & 800  & 100  & 100 \\
 & sci.med   & 800  & 100  & 100 \\
\midrule
 6 & sci.space   & 800  & 100  & 100 \\
 & misc.forsale   & 800  & 100  & 100 \\
\midrule
 7 & talk.politics.misc   & 800  & 100  & 100 \\
 & talk.politics.guns   & 800  & 100  & 100 \\
\midrule
 8 & talk.politics.mideast   & 800  & 100  & 100 \\
 & talk.religion.misc   & 800  & 100  & 100 \\
\midrule
 9 & alt.atheism   & 800  & 100  & 100 \\
 & soc.religion.christian   & 797  & 100  & 100 \\
 \bottomrule
\end{tabular}
}
\caption{Newsgroup dataset - class incremental}
\label{tab:data-newsgroup}
\end{table*}


\begin{table*}[]
\centering
\scalebox{0.8}{
\begin{tabular}{lrrr}
 \toprule
 Language &  train sents & dev sents & test sents \\
\midrule
  bn    &  15300  &  800  &  133119 \\
  de    &  15300  &  800  &  217824 \\
  en    &  15300  &  800  &  217818 \\
  es    &  15300  &  800  &  217887 \\
  fa    &  15300  &  800  &  165702 \\
  hi    &  15300  &  800  &  141565 \\
  ko    &  15300  &  800  &  178249 \\
  nl    &  15300  &  800  &  217337 \\
  ru    &  15300  &  800  &  217501 \\
  tr    &  15300  &  800  &  136935 \\
  zh    &  15300  &  800  &  151661 \\
 \bottomrule
\end{tabular}
}
\caption{MultcoNER dataset - Language incremental}
\label{tab:data-multiconer}
\end{table*}

\begin{table*}[]
\centering
\scalebox{0.8}{
\begin{tabular}{lrrrr}
 \hline
 Tasks & num tags & train sents & dev sents & test sents \\
 \hline
  action\_figures  & 15 & 2674 & 573 & 573 \\
camera\_lenses\_filters & 29 & 1309 & 280 & 282 \\
cell\_phones\_smartphones & 28 & 1044 & 223 & 225 \\
digital\_cameras & 24 & 700 & 150 & 150 \\
fine\_jewelry & 22 & 2634 & 564 & 566 \\
hunting & 20 & 1202 & 257 & 259 \\
kitchen\_dining\_bar & 12 & 1070 & 229 & 230 \\
tablets\_ebook\_readers & 32 & 1269 & 272 & 273 \\
womens\_shoes & 18 & 1040 & 222 & 224 \\
mixed & 79 & 12942 & 2770 & 2782 \\
 \hline
\end{tabular}
}
\caption{glue-ebay NER data statistics. The dataset contains 9 tasks with different number of NER tags. Mixed is the combined dataset of all 9 tasks with a universal tag set. Common tags across tasks are: O, brand, unit\_of\_measure, location, material, product\_name\_series}
\label{tab:ner-data}
\end{table*}

\begin{table*}[]
\centering
\scalebox{0.8}{
\begin{tabular}{lrrrr}
 \toprule
 Tasks & Class &  train sents & dev sents & test sents \\
\midrule
 0 & Know & 667 & 133 & 200\\
 & Warning & 146 & 30 & 44\\
 & Catastrophe & 667 & 133 & 200\\
 & Placing & 543 & 109 & 163\\
 & Causation & 667 & 133 & 200\\
 & Arriving & 667 & 133 & 200\\
 & Sending & 341 & 69 & 102\\
 & Protest & 123 & 25 & 37\\
 & Preventing or letting & 638 & 129 & 191\\
 & Motion & 667 & 133 & 200\\
 \midrule
 1 & Damaging & 667 & 133 & 200\\
 & Destroying & 667 & 133 & 200\\
 & Death & 667 & 133 & 200\\
 & Perception active & 285 & 58 & 85\\
 & Presence & 617 & 124 & 185\\
 & Influence & 541 & 109 & 162\\
 & Receiving & 241 & 49 & 72\\
 & Check & 198 & 41 & 59\\
 & Hostile encounter & 667 & 133 & 200\\
 & Killing & 667 & 133 & 200\\
 \midrule
 2 & Conquering & 667 & 133 & 200\\
 & Releasing & 95 & 20 & 28\\
 & Attack & 667 & 133 & 200\\
 & Earnings and losses & 667 & 133 & 200\\
 & Choosing & 379 & 77 & 113\\
 & Traveling & 624 & 126 & 187\\
 & Recovering & 224 & 46 & 67\\
 & Using & 408 & 82 & 122\\
 & Coming to be & 667 & 133 & 200\\
 & Cause to be included & 566 & 114 & 170\\
  \midrule
 3 & Process start & 667 & 133 & 200\\
 & Change event time & 214 & 43 & 64\\
 & Reporting & 385 & 78 & 115\\
 & Bodily harm & 667 & 133 & 200\\
 & Suspicion & 18 & 4 & 5\\
 & Statement & 667 & 133 & 200\\
 & Cause change of position on a scale & 667 & 133 & 200\\
 & Coming to believe & 170 & 34 & 51\\
 & Expressing publicly & 504 & 101 & 151\\
 & Request & 498 & 100 & 149\\
  \midrule
 4 & Control & 667 & 133 & 200\\
 & Supporting & 453 & 91 & 136\\
 & Defending & 615 & 124 & 184\\
 & Building & 283 & 57 & 85\\
 & Military operation & 667 & 133 & 200\\
 & Self motion & 667 & 133 & 200\\
 & GetReady & 84 & 17 & 25\\
 & Forming relationships & 82 & 17 & 24\\
 & Becoming a member & 192 & 40 & 57\\
 & Action & 576 & 116 & 172\\
  \midrule
 5 & Removing & 436 & 88 & 131\\
 & Surrendering & 164 & 33 & 49\\
 & Agree or refuse to act & 436 & 88 & 131\\
 & Participation & 564 & 114 & 169\\
 & Deciding & 289 & 59 & 86\\
 & Education teaching & 88 & 18 & 26\\
 & Emptying & 102 & 21 & 30\\
 & Getting & 667 & 133 & 200\\
 & Besieging & 208 & 42 & 62\\
 & Creating & 667 & 133 & 200\\
  \midrule
 6 & Process end & 667 & 133 & 200\\
 & Body movement & 93 & 19 & 28\\
 & Expansion & 216 & 44 & 65\\
 & Telling & 130 & 26 & 39\\
 & Change & 564 & 113 & 169\\
 & Legal rulings & 160 & 33 & 48\\
 & Bearing arms & 76 & 16 & 23\\
 & Giving & 463 & 93 & 139\\
 & Name conferral & 506 & 102 & 152\\
 & Arranging & 667 & 133 & 200\\
  \midrule
 7 & Use firearm & 358 & 73 & 107\\
 & Committing crime & 176 & 36 & 53\\
 & Assistance & 311 & 63 & 93\\
 & Surrounding & 83 & 17 & 25\\
 & Quarreling & 143 & 29 & 43\\
 & Expend resource & 72 & 15 & 21\\
 & Motion directional & 579 & 117 & 173\\
 & Bringing & 337 & 68 & 101\\
 & Communication & 388 & 78 & 116\\
 & Containing & 46 & 10 & 14\\
  \midrule
 8 & Manufacturing & 274 & 55 & 82\\
 & Social event & 667 & 133 & 200\\
 & Robbery & 46 & 10 & 14\\
 & Competition & 667 & 133 & 200\\
 & Writing & 80 & 16 & 24\\
 & Rescuing & 108 & 22 & 32\\
 & Judgment communication & 511 & 103 & 153\\
 & Hold & 667 & 133 & 200\\
 & Being in operation & 165 & 34 & 49\\
 & Recording & 436 & 88 & 131\\
  \midrule
 9 & Carry goods & 41 & 9 & 12\\
 & Cost & 69 & 15 & 20\\
 & Departing & 325 & 66 & 97\\
 & GiveUp & 138 & 28 & 41\\
 & Change of leadership & 622 & 125 & 186\\
 & Escaping & 637 & 128 & 191\\
 & Aiming & 231 & 47 & 69\\
 & Hindering & 238 & 48 & 71\\
 & Preserving & 148 & 30 & 44\\
 & Create artwork & 58 & 12 & 17\\
  \midrule
 10 & Openness & 180 & 37 & 54\\
 & Connect & 167 & 34 & 50\\
 & Reveal secret & 82 & 18 & 24\\
 & Response & 234 & 47 & 70\\
 & Scrutiny & 216 & 44 & 65\\
 & Lighting & 29 & 7 & 8\\
 & Criminal investigation & 184 & 38 & 55\\
 & Hiding objects & 82 & 17 & 24\\
 & Confronting problem & 150 & 30 & 45\\
 & Renting & 14 & 3 & 4\\
  \midrule
 11 & Patrolling & 72 & 15 & 21\\
 & Arrest & 252 & 52 & 75\\
 & Convincing & 137 & 28 & 41\\
 & Commerce sell & 102 & 21 & 30\\
 & Cure & 58 & 13 & 17\\
 & Temporary stay & 138 & 28 & 41\\
 & Dispersal & 284 & 57 & 85\\
 & Collaboration & 181 & 37 & 54\\
 & Change sentiment & 134 & 27 & 40\\
 & Commitment & 106 & 22 & 32\\
  \midrule
 12 & Commerce pay & 76 & 16 & 22\\
 & Filling & 79 & 17 & 23\\
 & Becoming & 667 & 133 & 200\\
 & Achieve & 232 & 47 & 69\\
 & Practice & 30 & 7 & 9\\
 & Cause change of strength & 667 & 133 & 200\\
 & Supply & 412 & 83 & 123\\
 & Cause to amalgamate & 249 & 51 & 74\\
 & Scouring & 26 & 6 & 7\\
 & Violence & 279 & 57 & 83\\
  \midrule
 13 & Reforming a system & 76 & 16 & 23\\
 & Come together & 266 & 54 & 80\\
 & Wearing & 61 & 13 & 18\\
 & Cause to make progress & 298 & 61 & 89\\
 & Legality & 112 & 24 & 33\\
 & Employment & 104 & 21 & 31\\
 & Rite & 39 & 9 & 11\\
 & Publishing & 196 & 40 & 58\\
 & Adducing & 66 & 14 & 20\\
 & Exchange & 52 & 12 & 15\\
  \midrule
 14 & Ratification & 22 & 5 & 6\\
 & Sign agreement & 144 & 30 & 43\\
 & Commerce buy & 42 & 10 & 12\\
 & Imposing obligation & 50 & 10 & 15\\
 & Rewards and punishments & 70 & 15 & 21\\
 & Testing & 108 & 22 & 32\\
 & Ingestion & 15 & 4 & 4\\
 & Labeling & 28 & 7 & 8\\
 & Kidnapping & 72 & 16 & 21\\
 & Submitting documents & 38 & 9 & 11\\
  \midrule
 15 & Prison & 46 & 10 & 13\\
 & Justifying & 22 & 6 & 6\\
 & Terrorism & 206 & 42 & 61\\
 & Vocalizations & 16 & 4 & 5\\
 & Risk & 10 & 2 & 3\\
 & Resolve problem & 104 & 22 & 31\\
 & Revenge & 42 & 10 & 12\\
 & Limiting & 64 & 13 & 19\\
 & Research & 72 & 15 & 21\\
 & Having or lacking access & 53 & 11 & 16\\
  \midrule
 16 & Theft & 16 & 4 & 4\\
 & Incident & 11 & 3 & 3\\
 & Award & 47 & 10 & 14 \\
 \bottomrule
\end{tabular}
}
\caption{Maven dataset - Task incremental - 163 classes - 10 tasks.}
\label{tab:data-maven}
\end{table*}


==> tables/tab-result-asc.tex <==
\begin{table*}[]
\centering
 \caption{Average accuracy (6 runs or task orders) and standard deviation of different ACL models at the end of tasks on ASC dataset. The columns show the non-CL algorithms: individual learning (\textsc{Indiv}) and multi-task learning (\textsc{Mtl}); and CL algorithms: finetuning (\textsc{Ft}), Elastic Weight Consolidation (\textsc{EWC}) and Experiment Replay (\textsc{ER}). The AL algorithms and theirs corresponding independent labelling are shown in the rows: random (\textsc{Rand}), entropy (\textsc{Ent}), min-margin (\textsc{Marg}), BADGE and embedding $k$-means (\textsc{kMeans}). The best score of each column and within the same ACL group are marked in \textbf{bold} and \underline{underline} respectively. $^\dagger$ denotes the best CL algorithm within the same AL strategy.}
\scalebox{0.75}{
    \begin{tabular}{l|ll|lll}
    \toprule
%    & \multicolumn{5}{c|}{ASC (Domain-IL)} & \multicolumn{5}{c}{Newsgroup (Class-IL)} \\
\multicolumn{1}{c|}{AL/CL} & \multicolumn{1}{c}{\textsc{Indiv}} & \multicolumn{1}{c|}{\textsc{Mtl}} & \multicolumn{1}{c}{\textsc{Ft}} & \multicolumn{1}{c}{EWC} & \multicolumn{1}{c}{ER}\\
\midrule
    \textsc{Full} & \textbf{92.36} $\scriptstyle\pm0.84$&95.00 $\scriptstyle\pm0.27$ &94.30 $\scriptstyle\pm1.09$&94.85$^\dagger\scriptstyle\pm1.00$&94.19 $\scriptstyle\pm1.21$\\
\midrule
\textsc{Ind. Rand}&&93.45 $\scriptstyle\pm0.47$&92.43 $\scriptstyle\pm1.26$&\underline{93.38} $\scriptstyle\pm0.79$&93.69$^\dagger\scriptstyle\pm0.99$\\
\textsc{Rand}&88.01 $\scriptstyle\pm1.78$&\underline{94.41} $\scriptstyle\pm0.80$&\underline{94.10}$^\dagger\scriptstyle\pm0.77$&93.03 $\scriptstyle\pm0.75$&\underline{93.71} $\scriptstyle\pm1.29$\\
\midrule
\textsc{Ind. Ent}&&\textbf{95.06} $\scriptstyle\pm0.19$&94.49 $\scriptstyle\pm0.82$&94.66 $\scriptstyle\pm0.95$&94.88$^\dagger\scriptstyle\pm0.91$\\
\textsc{Ent}&91.51 $\scriptstyle\pm0.84$&94.95 $\scriptstyle\pm0.58$&\underline{95.08} $\scriptstyle\pm0.52$&\underline{95.58}$^\dagger\scriptstyle\pm0.33$&\underline{95.07} $\scriptstyle\pm0.55$\\
\midrule
\textsc{Ind. Marg}&&\underline{94.95} $\scriptstyle\pm0.37$&94.38 $\scriptstyle\pm1.64$&94.32 $\scriptstyle\pm0.98$&94.73$^\dagger\scriptstyle\pm0.95$\\
\textsc{Marg}&91.75 $\scriptstyle\pm0.74$&94.49 $\scriptstyle\pm0.83$&\textbf{95.31 $\scriptstyle\pm0.55$}&\textbf{95.68}$^\dagger\scriptstyle\pm0.56$&\textbf{95.55 $\scriptstyle\pm0.38$}\\
\midrule
\textsc{Ind. BADGE}&&93.82 $\scriptstyle\pm0.54$&\underline{92.83} $\scriptstyle\pm1.17$&93.07 $\scriptstyle\pm0.50$&\underline{94.34}$^\dagger\scriptstyle\pm0.58$\\
\textsc{BADGE}&83.61 $\scriptstyle\pm3.23$&\underline{93.85} $\scriptstyle\pm0.42$&92.68 $\scriptstyle\pm1.11$&\underline{93.15} $\scriptstyle\pm0.42$&94.24$^\dagger\scriptstyle\pm0.49$\\
\midrule
\textsc{ind. kMeans}&&\underline{94.78} $\scriptstyle\pm0.32$&93.81 $\scriptstyle\pm1.39$&92.88 $\scriptstyle\pm1.56$&\underline{94.72}$^\dagger\scriptstyle\pm0.79$\\
\textsc{kMeans}&86.26 $\scriptstyle\pm2.42$&93.93 $\scriptstyle\pm0.60$&\underline{94.35}$^\dagger\scriptstyle\pm0.64$&\underline{93.59} $\scriptstyle\pm0.72$&93.76 $\scriptstyle\pm1.57$\\
    \bottomrule
\end{tabular}
}
   
\label{tab:asc-ret}
\end{table*}

==> tables/tab-result-newsgroup.tex <==
\begin{table*}[]
\centering
 \caption{Average accuracy (6 runs or task orders) and standard deviation of different ACL models at the end of tasks on 20News dataset in class-IL and task-IL settings.
%    The columns and rows presents the non-CL/CL and AL algorithms respectively. The best score of each column and within the same ACL group are marked in \textbf{bold} and \underline{underline} respectively. $^\dagger$ denotes the best CL algorithm within the same AL strategy.
    }
\scalebox{0.68}{
    \begin{tabular}{l|l|llll|llll}
    \toprule
    & &\multicolumn{4}{c|}{Class-IL} & \multicolumn{4}{c}{Task-IL} \\
\multicolumn{1}{c|}{AL/CL} & \multicolumn{1}{c|}{\textsc{Indiv}} & \multicolumn{1}{c}{\textsc{Mtl}} & \multicolumn{1}{c}{\textsc{Ft}} & \multicolumn{1}{c}{EWC} & \multicolumn{1}{c|}{ER} &  \multicolumn{1}{c}{\textsc{Mtl}} &\multicolumn{1}{c}{\textsc{Ft}} & \multicolumn{1}{c}{EWC} & \multicolumn{1}{c}{ER}   \\
\midrule
 \textsc{Full} & \textbf{91.78} $\scriptstyle\pm0.47$&\textbf{72.42} $\scriptstyle\pm0.62$ & \textbf{9.94} $\scriptstyle\pm0.88$& \textbf{9.32} $\scriptstyle\pm0.43$&55.15$^\dagger\scriptstyle\pm1.00$ & \textbf{91.17} $\scriptstyle\pm0.69$ &\textbf{70.48} $\scriptstyle\pm3.25$&\textbf{77.45} $\scriptstyle\pm1.56$&\textbf{89.33}$^\dagger\scriptstyle\pm0.62$\\
 \midrule
\textsc{Ind. Rand}&&67.07 $\scriptstyle\pm0.52$&8.87 $\scriptstyle\pm0.59$&\underline{9.00} $\scriptstyle\pm0.51$&\underline{56.15} $\scriptstyle\pm1.02$ &\underline{89.44} $\scriptstyle\pm0.54$&\underline{65.04}$\scriptstyle\pm1.74$&60.01 $\scriptstyle\pm5.45$&\underline{88.04}$^\dagger\scriptstyle\pm0.75$\\
\textsc{Rand}&88.95 $\scriptstyle\pm0.60$&\underline{67.33} $\scriptstyle\pm0.46$&\underline{8.90} $\scriptstyle\pm0.44$&8.99 $\scriptstyle\pm0.52$&55.25$^\dagger\scriptstyle\pm2.34$&89.27 $\scriptstyle\pm0.52$&63.34 $\scriptstyle\pm2.48$&\underline{63.23} $\scriptstyle\pm1.93$&87.81$^\dagger\scriptstyle\pm0.59$\\
\midrule
\textsc{Ind. Ent}&&63.61 $\scriptstyle\pm1.10$&8.75 $\scriptstyle\pm0.64$&8.86 $\scriptstyle\pm0.53$&\underline{54.74}$^\dagger\scriptstyle\pm2.90$&89.09 $\scriptstyle\pm0.70$&60.54 $\scriptstyle\pm2.84$&\underline{64.77} $\scriptstyle\pm5.02$&87.44$^\dagger\scriptstyle\pm0.58$\\
\textsc{Ent}&89.08 $\scriptstyle\pm0.58$&\underline{65.21} $\scriptstyle\pm0.88$&\underline{8.84} $\scriptstyle\pm0.61$&\underline{8.94} $\scriptstyle\pm0.48$&52.42$^\dagger\scriptstyle\pm1.42$&\underline{89.10} $\scriptstyle\pm0.46$&\underline{61.41} $\scriptstyle\pm4.81$&61.38 $\scriptstyle\pm7.03$&\underline{88.47}$^\dagger\scriptstyle\pm0.58$\\
\midrule
\textsc{Ind. Marg}&&64.78 $\scriptstyle\pm1.03$&8.87 $\scriptstyle\pm0.57$&\underline{9.19} $\scriptstyle\pm0.55$&\underline{55.07} $\scriptstyle\pm1.26$&88.78 $\scriptstyle\pm0.76$&\underline{63.46} $\scriptstyle\pm4.19$&\underline{63.76} $\scriptstyle\pm5.14$&88.23$^\dagger\scriptstyle\pm0.35$\\
\textsc{Marg}&90.38 $\scriptstyle\pm0.64$&\underline{67.66} $\scriptstyle\pm0.47$&\underline{8.95} $\scriptstyle\pm0.55$&9.05 $\scriptstyle\pm0.58$&52.83$^\dagger\scriptstyle\pm2.24$&\underline{89.80} $\scriptstyle\pm0.38$&62.41 $\scriptstyle\pm2.63$&61.18 $\scriptstyle\pm2.38$&\underline{88.65}$^\dagger\scriptstyle\pm0.23$\\
\midrule
\textsc{Ind. BADGE}&&67.27 $\scriptstyle\pm0.65$&\underline{8.96} $\scriptstyle\pm0.47$&8.85 $\scriptstyle\pm0.52$&\underline{57.11}$^\dagger\scriptstyle\pm1.10$&89.08 $\scriptstyle\pm0.37$&{63.76} $\scriptstyle\pm2.56$&\underline{67.30} $\scriptstyle\pm4.70$&87.67$^\dagger\scriptstyle\pm0.85$\\
\textsc{BADGE}&88.74 $\scriptstyle\pm0.40$&\underline{67.64} $\scriptstyle\pm0.54$&8.95 $\scriptstyle\pm0.48$&\underline{8.94} $\scriptstyle\pm0.47$&54.60$^\dagger\scriptstyle\pm2.13$&\underline{89.52} $\scriptstyle\pm0.84$&\underline{64.92} $\scriptstyle\pm1.72$&64.16 $\scriptstyle\pm3.42$&\underline{88.05}$^\dagger\scriptstyle\pm0.54$\\
\midrule
\textsc{ind. kMeans}&&66.60 $\scriptstyle\pm0.77$&9.28 $\scriptstyle\pm0.95$&\underline{8.94} $\scriptstyle\pm0.50$&\textbf{57.32}$^\dagger\scriptstyle\pm1.86$&88.91 $\scriptstyle\pm0.47$&65.66 $\scriptstyle\pm2.88$&\underline{67.69} $\scriptstyle\pm4.09$&87.82$^\dagger\scriptstyle\pm0.56$\\
\textsc{kMeans}&88.67 $\scriptstyle\pm0.74$&\underline{67.41} $\scriptstyle\pm0.68$&\underline{9.49} $\scriptstyle\pm1.33$&8.88 $\scriptstyle\pm0.50$&54.54$^\dagger\scriptstyle\pm2.38$&\underline{89.23} $\scriptstyle\pm0.45$&\underline{68.32} $\scriptstyle\pm1.98$&64.04 $\scriptstyle\pm3.75$&\underline{87.47}$^\dagger\scriptstyle\pm1.08$\\
    \bottomrule
\end{tabular}
}
   
\label{tab:newsgroup-ret}
\end{table*}

==> tables/tab-result-seq-mnist.tex <==
\begin{table*}[]
\centering
 \caption{Average accuracy (6 runs or task orders) and standard deviation of different ACL models at the end of tasks on sequential MNIST dataset in class-IL and task-IL settings. The best ACL score in each column is marked in \textbf{bold}. $^\dagger$ denotes the best CL algorithm within the same AL strategy.
%    The columns and rows presents the non-CL/CL and AL algorithms respectively. The best score of each column and within the same ACL group are marked in \textbf{bold} and \underline{underline} respectively. $^\dagger$ denotes the best CL algorithm within the same AL strategy.
    }
\scalebox{0.75}{
    \begin{tabular}{l|l|llll|llll}
    \toprule
    & &\multicolumn{4}{c|}{Class-IL} & \multicolumn{4}{c}{Task-IL} \\
\multicolumn{1}{c|}{AL/CL} & \multicolumn{1}{c|}{\textsc{Indiv}} & \multicolumn{1}{c}{\textsc{Mtl}} & \multicolumn{1}{c}{\textsc{Ft}} & \multicolumn{1}{c}{EWC} & \multicolumn{1}{c|}{ER} & \multicolumn{1}{c}{\textsc{Mtl}} & \multicolumn{1}{c}{\textsc{Ft}} & \multicolumn{1}{c}{EWC} & \multicolumn{1}{c}{ER}   \\
\midrule
 \textsc{Full} & 99.60 $\scriptstyle\pm0.03$&96.64 $\scriptstyle\pm0.28$ &19.93 $\scriptstyle\pm0.05$&19.98 $\scriptstyle\pm0.06$&77.66 $\scriptstyle\pm3.09$&
 99.36 $\scriptstyle\pm0.05$ &59.45 $\scriptstyle\pm4.40$&74.17 $\scriptstyle\pm5.51$&96.45 $\scriptstyle\pm1.15$\\
\midrule
% \textsc{Ind. Rand}&&\\
\textsc{Rand}&\textbf{99.66} $\scriptstyle\pm0.08$&94.36 $\scriptstyle\pm0.78$&19.98 $\scriptstyle\pm0.06$&20.25 $\scriptstyle\pm0.41$&75.37$^\dagger\scriptstyle\pm2.91$&99.02 $\scriptstyle\pm0.11$&\textbf{66.02} $\scriptstyle\pm7.25$&68.04 $\scriptstyle\pm7.24$&95.70$^\dagger\scriptstyle\pm0.79$\\
% \midrule
% \textsc{Ind. Ent}&&\\
\textsc{Ent}&99.61 $\scriptstyle\pm0.06$&96.01 $\scriptstyle\pm0.23$&19.97 $\scriptstyle\pm0.02$&20.04 $\scriptstyle\pm0.12$&77.60$^\dagger\scriptstyle\pm4.51$&
99.37 $\scriptstyle\pm0.09$&57.46 $\scriptstyle\pm6.72$&70.46$^\dagger\scriptstyle\pm5.72$&96.41$^\dagger\scriptstyle\pm0.65$\\
% \midrule
% \textsc{Ind. Marg}&&\\
\textsc{Marg}&99.62 $\scriptstyle\pm0.06$&\textbf{96.34} $\scriptstyle\pm0.31$&19.95 $\scriptstyle\pm0.03$&\textbf{20.53} $\scriptstyle\pm0.76$&77.71$^\dagger\scriptstyle\pm4.59$&\textbf{99.51} $\scriptstyle\pm0.06$&57.46 $\scriptstyle\pm6.72$&\textbf{71.30} $\scriptstyle\pm6.07$&\textbf{96.42}$^\dagger\scriptstyle\pm0.35$\\
% \midrule
% \textsc{Ind. BADGE}&&\\
\textsc{BADGE}&99.62 $\scriptstyle\pm0.04$&93.72 $\scriptstyle\pm0.65$&19.96 $\scriptstyle\pm0.02$&20.12 $\scriptstyle\pm0.23$&76.87$^\dagger\scriptstyle\pm2.53$&
98.88 $\scriptstyle\pm0.18$&61.49 $\scriptstyle\pm5.54$&70.37 $\scriptstyle\pm5.67$&96.11$^\dagger\scriptstyle\pm0.72$\\
% \midrule
% \textsc{ind. coreset}&&\\
\textsc{Coreset}&99.61 $\scriptstyle\pm0.03$&96.05 $\scriptstyle\pm0.27$&\textbf{20.00} $\scriptstyle\pm0.05$&19.99 $\scriptstyle\pm0.02$&\textbf{78.18}$^\dagger\scriptstyle\pm2.96$&
99.45 $\scriptstyle\pm0.08$&63.88 $\scriptstyle\pm5.19$&65.77 $\scriptstyle\pm6.94$&95.96$^\dagger\scriptstyle\pm0.35$\\
    \bottomrule
\end{tabular}
}
\label{tab:mnist-ret}
\end{table*}



==> tables/tab-result.tex <==
\begin{table*}[]
\centering
\scalebox{0.65}{
    \begin{tabular}{llllll|llllll}
    \toprule
    & \multicolumn{5}{c|}{ASC (Domain-IL)} & \multicolumn{5}{c}{Newsgroup (Class-IL)} \\
\multicolumn{1}{c}{AL/CL} & \multicolumn{1}{c}{\textsc{Indiv}} & \multicolumn{1}{c}{\textsc{Mtl}} & \multicolumn{1}{c}{\textsc{Ft}} & \multicolumn{1}{c}{EWC} & \multicolumn{1}{c|}{ER} &\multicolumn{1}{c}{\textsc{Indiv}} & \multicolumn{1}{c}{\textsc{Mtl}} & \multicolumn{1}{c}{\textsc{Ft}} & \multicolumn{1}{c}{EWC} & \multicolumn{1}{c}{ER}   \\
\midrule
    \textsc{Full} & 92.36 $\scriptstyle\pm0.84$&95.00 $\scriptstyle\pm0.27$ &94.30 $\scriptstyle\pm1.09$&94.85 $\scriptstyle\pm1.00$&94.19 $\scriptstyle\pm1.21$&  91.78 $\scriptstyle\pm0.47$&72.42 $\scriptstyle\pm0.62$ &9.94 $\scriptstyle\pm0.88$&9.32 $\scriptstyle\pm0.43$&55.15 $\scriptstyle\pm1.00\\
\midrule
\textsc{Ind. Rand}&&93.45 $\scriptstyle\pm0.47$&92.43 $\scriptstyle\pm1.26$&93.38 $\scriptstyle\pm0.79$&93.69 $\scriptstyle\pm0.99$&&67.07 $\scriptstyle\pm0.52$&8.87 $\scriptstyle\pm0.59$&9.25 $\scriptstyle\pm0.32$&55.52 $\scriptstyle\pm1.00$\\
\textsc{Rand}&88.01 $\scriptstyle\pm1.78$&94.41 $\scriptstyle\pm0.80$&94.10 $\scriptstyle\pm0.77$&93.03 $\scriptstyle\pm0.75$&93.71 $\scriptstyle\pm1.29$&88.95 $\scriptstyle\pm0.60$&67.33 $\scriptstyle\pm0.46$&8.90 $\scriptstyle\pm0.44$&8.99 $\scriptstyle\pm0.52$&55.25 $\scriptstyle\pm2.34$\\
\midrule
\textsc{Ind. Ent}&&95.06 $\scriptstyle\pm0.19$&94.49 $\scriptstyle\pm0.82$&94.66 $\scriptstyle\pm0.95$&94.88 $\scriptstyle\pm0.91$&&63.61 $\scriptstyle\pm1.10$&8.89 $\scriptstyle\pm0.62$&8.75 $\scriptstyle\pm0.52$&52.42 $\scriptstyle\pm1.42$\\
\textsc{Ent}&91.51 $\scriptstyle\pm0.84$&94.95 $\scriptstyle\pm0.58$&95.08 $\scriptstyle\pm0.52$&95.58 $\scriptstyle\pm0.33$&95.07 $\scriptstyle\pm0.55$&89.08 $\scriptstyle\pm0.58$&65.21 $\scriptstyle\pm0.88$&8.84 $\scriptstyle\pm0.61$&8.94 $\scriptstyle\pm0.48$&54.40 $\scriptstyle\pm3.06$\\
\midrule
\textsc{Ind. Marg}&&94.95 $\scriptstyle\pm0.37$&94.38 $\scriptstyle\pm1.64$&94.32 $\scriptstyle\pm0.98$&94.73 $\scriptstyle\pm0.95$&&64.78 $\scriptstyle\pm1.03$&8.87 $\scriptstyle\pm0.57$&9.09 $\scriptstyle\pm0.54$&52.83 $\scriptstyle\pm2.24$\\
\textsc{Marg}&91.75 $\scriptstyle\pm0.74$&94.49 $\scriptstyle\pm0.83$&95.31 $\scriptstyle\pm0.55$&95.68 $\scriptstyle\pm0.56$&95.55 $\scriptstyle\pm0.38$&90.38 $\scriptstyle\pm0.64$&67.66 $\scriptstyle\pm0.47$&8.95 $\scriptstyle\pm0.55$&9.05 $\scriptstyle\pm0.58$&54.54 $\scriptstyle\pm0.27$\\
\midrule
\textsc{Ind. BADGE}&&93.82 $\scriptstyle\pm0.54$&92.83 $\scriptstyle\pm1.17$&93.07 $\scriptstyle\pm0.50$&94.34 $\scriptstyle\pm0.58$&&67.27 $\scriptstyle\pm0.65$&8.96 $\scriptstyle\pm0.47$&8.85 $\scriptstyle\pm0.52$&54.60 $\scriptstyle\pm2.13$\\
\textsc{BADGE}&83.61 $\scriptstyle\pm3.23$&93.85 $\scriptstyle\pm0.42$&92.68 $\scriptstyle\pm1.11$&93.15 $\scriptstyle\pm0.42$&94.24 $\scriptstyle\pm0.49$&88.74 $\scriptstyle\pm0.40$&67.64 $\scriptstyle\pm0.54$&8.95 $\scriptstyle\pm0.48$&8.94 $\scriptstyle\pm0.47$&57.19 $\scriptstyle\pm1.16$\\
\midrule
\textsc{ind. kMeans}&&94.78 $\scriptstyle\pm0.32$&93.81 $\scriptstyle\pm1.39$&92.88 $\scriptstyle\pm1.56$&94.72 $\scriptstyle\pm0.79$&&66.60 $\scriptstyle\pm0.77$&9.28 $\scriptstyle\pm0.95$&8.98 $\scriptstyle\pm0.53$&54.54 $\scriptstyle\pm2.38$\\
\textsc{kMeans}&86.26 $\scriptstyle\pm2.42$&93.93 $\scriptstyle\pm0.60$&94.35 $\scriptstyle\pm0.64$&93.59 $\scriptstyle\pm0.72$&93.76 $\scriptstyle\pm1.57$&88.67 $\scriptstyle\pm0.74$&67.41 $\scriptstyle\pm0.68$&9.49 $\scriptstyle\pm1.33$&8.88 $\scriptstyle\pm0.50$&57.29 $\scriptstyle\pm2.04$\\
    \bottomrule
\end{tabular}
}
    \caption{Average accuracy (6 runs or task orders) and standard deviation of different ACL models on ASC and 20News tasks. The columns show the non-CL algorithms: individual learning (\textsc{Indiv}) and multi-task learning (\textsc{Mtl}); and CL algorithms: finetuning (\textsc{Ft}), Elastic Weight Consolidation (\textsc{EWC}) and Experiment Replay (\textsc{ER}). The AL algorithms and theirs corresponding independent labelling are shown in the rows: random (\textsc{Rand}), entropy (\textsc{Ent}), min-margin (\textsc{Marg}), BADGE and embedding $k$-means (\textsc{kMeans}). \trang{imcomplete results - missing some runs}}
\label{tab:main-ret}
\end{table*}
